A first look into the carbon footprint of federated learning

Despite impressive results, deep learning-based technologies also raise severe privacy and environmental concerns induced by the training procedure often conducted in data centers. In response, alternatives to centralized training such as Federated Learning (FL) have emerged. Perhaps unexpectedly, FL is starting to be deployed at a global scale by companies that must adhere to new legal demands and policies originating from governments and social groups advocating for privacy protection. \textit{However, the potential environmental impact related to FL remains unclear and unexplored. This paper offers the first-ever systematic study of the carbon footprint of FL.} First, we propose a rigorous model to quantify the carbon footprint, hence facilitating the investigation of the relationship between FL design and carbon emissions. Then, we compare the carbon footprint of FL to traditional centralized learning. Our findings show that, depending on the configuration, FL can emit up to two order of magnitude more carbon than centralized machine learning. However, in certain settings, it can be comparable to centralized learning due to the reduced energy consumption of embedded devices. We performed extensive experiments across different types of datasets, settings and various deep learning models with FL. Finally, we highlight and connect the reported results to the future challenges and trends in FL to reduce its environmental impact, including algorithms efficiency, hardware capabilities, and stronger industry transparency.

==> 2.2_motivation.tex <==
\section{Federated Learning and the Environment}
Federated learning provides many advantages when compared to centralized learning. At present, data owners are holding more and more sensitive information, such as individual activity data, life-logging videos, email conversations, and others \citep{fedcs}. For example, keeping personal medical and healthcare data private recently became one of the major ethical concerns \citep{kish2015unpatients}. To this extent, and in response to an increasing number of such privacy issues, policymakers have responded with the implementation of data privacy legislation such as the European General Data Protection Regulation (GDPR) \citep{lim2020federated}. Due to these regulations, moving data across national borders becomes subject to data sovereignty law, making centralized training infeasible in some scenarios \citep{hsieh2019non}.

Furthermore, there are nearly seven billion connected Internet of Things (IoT) devices \citep{lim2020federated} and three billion smartphones around the world, potentially giving access to an astonishing amount of training data and compute power for meaningful research and applications. Using mobile sensing and smartphones to boost large-scale health studies, such as in \citet{7167448}, \citet{9106648} and \citet{shen2015smartphones}, has caused increased interest in the healthcare research field, and privacy-friendly framework including FL are potential solutions to answer this demand.

Whilst the carbon footprint for centralized learning has been studied in many previous works \citep{anthony2020carbontracker,lacoste2019quantifying,henderson2020towards,uchechukwu2014energy}, the energy consumption and carbon footprint related to FL remain unexplored. To this extent, this paper proposes to overcome this issue by giving a first look into the carbon analysis of FL. State-of-the-art results in deep learning are usually determined by metrics such as the accuracy of a given model or model size, while energy efficiency or privacy concerns are often overlooked. Whilst accuracy remains crucial, we hope to encourage researchers to also focus on other metrics that are in line with the increasing interest of the civil society for global warming. By quantifying carbon emissions for FL and demonstrating that very specific FL setups may lead to a decrease of these emissions, we encourage the integration of the released CO$_2$e as a crucial metric to the FL deployment.  

%\newpage

%As an example, in the case of non-sensitive datasets, researchers are free to choose between centralised training and FL. However, sensitive data including personal information or medical details force researchers to take extra care while manipulating and training models based on these data.  

%However, when dealing with more sensitive datasets, such as datasets that involves personal information or medical details, researchers are required to take extra care during training and FL can be more favorable than centralised training. There are also cases when both centralised training and FL can be involved. By using this kind of ``hybrid" training, researchers can process the sensitive part federatedly while training the non-sensitive part in the centralised way. In this way, details comparison between centralised training and FL are needed, hence interested researchers are able to make informed decisions in the optimal way.%interested researchers are able to make informed decisions between centralised learning and FL based on the different scenarios. 

==> 7.2_graph.tex <==
\begin{figure*}[!t]
\centering
\begin{tabular}{P{5cm}P{5cm}}

\begin{tikzpicture}[scale = 0.55]
\pgfplotsset{
      scale only axis,
  }

  \begin{axis}[
    xlabel=CO$_2$e emitted in g. (IID and 5 local epoch),
    ylabel=Accuracy in $\%$,
    xmin=20,   % start the diagram at this x-coordinate
    xmax=120,  % end  the diagram at this x-coordinate
    ymin=0.55,   % start the diagram at this y-coordinate
    ymax=0.75,
    legend style={at={(1.15,1.2)},anchor=north, legend columns=5}
  ]
    \addplot[only marks, mark options={scale=1.5}, mark=x]
    coordinates{ % plot 1 data set
      (97.64,0.686)
      % more points...
    }; \label{plot_one}
    % plot 1 legend entry
    %\addlegendimage{/pgfplots/refstyle=plot_one}
    \addlegendentry{1 client }
    
     \addplot[only marks, mark options={scale=1.5}, mark=o]
    coordinates{ % plot 1 data set
      (64.05,0.66)
      % more points...
    }; \label{plot_two}
    \addlegendentry{2 clients }
    %\addlegendimage{/pgfplots/refstyle=plot_two}
    
     \addplot[only marks, mark options={scale=1.5}, mark=*]
    coordinates{ % plot 1 data set
      (58.58,0.653)
      % more points...
    }; \label{plot_three}
    \addlegendentry{3 clients }
    
    \addplot[only marks, mark options={scale=1.5}, mark=square*]
    coordinates{ % plot 1 data set
      (62.49,0.66)
      % more points...
    }; \label{plot_four}
    \addlegendentry{4 clients }
    
    \addplot[only marks, mark options={scale=1.5}, mark=diamond*]
    coordinates{ % plot 1 data set
      (68.35,0.65)
      % more points...
    }; 
    \addlegendentry{5 clients }
    
     \addplot[only marks, mark options={scale=1.5}, mark=triangle*]
    coordinates{ % plot 1 data set
      (42.18,0.645)
      % more points...
    };
    \addlegendentry{6 clients }
    
    \addplot[only marks, mark options={scale=1.5}, mark=star]
    coordinates{ % plot 1 data set
      (41.01,0.645)
      % more points...
    }; 
    \addlegendentry{7 clients }
    
    
    \addplot[only marks, mark options={scale=1.5}, mark=+]
    coordinates{ % plot 1 data set
      (49.99,0.645)
      % more points...
    };
    \addlegendentry{8 clients }
    
    \addplot[only marks, mark options={scale=1.5}, mark=triangle]
    coordinates{ % plot 1 data set
      (56.24,0.645)
      % more points...
    };
    \addlegendentry{9 clients }
    
    \addplot[only marks, mark options={scale=1.5}, mark=square]
    coordinates{ % plot 1 data set
      (70.3,0.645)
      % more points...
    };
    \addlegendentry{10 client }
  \end{axis}

\end{tikzpicture}

&

\begin{tikzpicture}[scale = 0.55]
\pgfplotsset{
      scale only axis,
  }

  \begin{axis}[
   xlabel=CO$_2$e emitted in g. (non-IID and 5 local epoch),
    ylabel=Accuracy in $\%$,
    xmin=20,   % start the diagram at this x-coordinate
    xmax=150,  % end  the diagram at this x-coordinate
    ymin=0.55,   % start the diagram at this y-coordinate
    ymax=0.75,
    %legend style={at={(0.5,1.1)},anchor=north, legend columns=-1}
  ]
    \addplot[only marks, mark options={scale=1.5}, mark=x]
    coordinates{ % plot 1 data set
      (97.64,0.655)
    }; \label{plot_one}

 
     \addplot[only marks, mark options={scale=1.5}, mark=o]
    coordinates{ % plot 1 data set
      (148.41,0.653)
    }; \label{plot_two}

    
     \addplot[only marks, mark options={scale=1.5}, mark=*]
    coordinates{ % plot 1 data set
      (105.45,0.647)
    }; \label{plot_three}

    
    \addplot[only marks, mark options={scale=1.5}, mark=square*]
    coordinates{ % plot 1 data set
      (78.11,0.637)
    }; \label{plot_four}

    
    \addplot[only marks, mark options={scale=1.5}, mark=diamond*]
    coordinates{ % plot 1 data set
      (78.11,0.635)
    }; 

    
     \addplot[only marks, mark options={scale=1.5}, mark=triangle*]
    coordinates{ % plot 1 data set
      (93.7,0.635)
    };

    
    \addplot[only marks, mark options={scale=1.5}, mark=star]
    coordinates{ % plot 1 data set
      (109.36,0.635)
    }; 

    
    
    \addplot[only marks, mark options={scale=1.5}, mark=+]
    coordinates{ % plot 1 data set
      (59.37,0.62)
    };

    
    \addplot[only marks, mark options={scale=1.5}, mark=triangle]
    coordinates{ % plot 1 data set
      (59.76,0.62)
    }; 

    
    \addplot[only marks, mark options={scale=1.5}, mark=square]
    coordinates{ % plot 1 data set
      (54.68,0.623)
    }; 

  \end{axis}

\end{tikzpicture}

\\

\begin{tikzpicture}[scale = 0.55]
\pgfplotsset{
      scale only axis,
  }

  \begin{axis}[
    xlabel=CO$_2$e emitted in g. (IID and 1 local epoch),
    ylabel=Accuracy in $\%$,
    xmin=20,   % start the diagram at this x-coordinate
    xmax=120,  % end  the diagram at this x-coordinate
    ymin=0.55,   % start the diagram at this y-coordinate
    ymax=0.75,
    %legend style={at={(0.5,1.1)},anchor=north, legend columns=-1}
  ]
    \addplot[only marks, mark options={scale=1.5}, mark=x]
    coordinates{ % plot 1 data set
      (25.78,0.702)
    }; \label{plot_one}

 
     \addplot[only marks, mark options={scale=1.5}, mark=o]
    coordinates{ % plot 1 data set
      (31.25,0.67)
    }; \label{plot_two}

    
     \addplot[only marks, mark options={scale=1.5}, mark=*]
    coordinates{ % plot 1 data set
      (23.43,0.66)
    }; \label{plot_three}

    
    \addplot[only marks, mark options={scale=1.5}, mark=square*]
    coordinates{ % plot 1 data set
      (21.87,0.64)
    }; \label{plot_four}

    
    \addplot[only marks, mark options={scale=1.5}, mark=diamond*]
    coordinates{ % plot 1 data set
      (28.51,0.643)
    }; 

    
     \addplot[only marks, mark options={scale=1.5}, mark=triangle*]
    coordinates{ % plot 1 data set
      (31.87,0.637)
    };

    
    \addplot[only marks, mark options={scale=1.5}, mark=star]
    coordinates{ % plot 1 data set
      (33.35,0.627)
    }; 

    
    
    \addplot[only marks, mark options={scale=1.5}, mark=+]
    coordinates{ % plot 1 data set
      (34.37,0.630)
    };

    
    \addplot[only marks, mark options={scale=1.5}, mark=triangle]
    coordinates{ % plot 1 data set
      (28.12,0.63)
    }; 

    
    \addplot[only marks, mark options={scale=1.5}, mark=square]
    coordinates{ % plot 1 data set
      (35.15,0.625)
    }; 

  \end{axis}

\end{tikzpicture}

&

\begin{tikzpicture}[scale = 0.55]
\pgfplotsset{
      scale only axis,
  }

  \begin{axis}[
    xlabel=CO$_2$e emitted in g. (non-IID and 1 local epoch),
    ylabel=Accuracy in $\%$,
    xmin=20,   % start the diagram at this x-coordinate
    xmax=120,  % end  the diagram at this x-coordinate
    ymin=0.55,   % start the diagram at this y-coordinate
    ymax=0.75,
    %legend style={at={(0.5,1.1)},anchor=north, legend columns=-1}
  ]
    \addplot[only marks, mark options={scale=1.5}, mark=x]
    coordinates{ % plot 1 data set
      (35.15,0.668)
    }; \label{plot_one}

 
     \addplot[only marks, mark options={scale=1.5}, mark=o]
    coordinates{ % plot 1 data set
      (51.55,0.645)
    }; \label{plot_two}

    
     \addplot[only marks, mark options={scale=1.5}, mark=*]
    coordinates{ % plot 1 data set
      (70.30,0.628)
    }; \label{plot_three}

    
    \addplot[only marks, mark options={scale=1.5}, mark=square*]
    coordinates{ % plot 1 data set
      (49.99,0.628)
    }; \label{plot_four}

    
    \addplot[only marks, mark options={scale=1.5}, mark=diamond*]
    coordinates{ % plot 1 data set
      (54.68,0.61)
    }; 

    
     \addplot[only marks, mark options={scale=1.5}, mark=triangle*]
    coordinates{ % plot 1 data set
      (60.93,0.615)
    };

    
    \addplot[only marks, mark options={scale=1.5}, mark=star]
    coordinates{ % plot 1 data set
      (32.81,0.600)
    }; 

    
    
    \addplot[only marks, mark options={scale=1.5}, mark=+]
    coordinates{ % plot 1 data set
      (37.49,0.590)
    };

    
    \addplot[only marks, mark options={scale=1.5}, mark=triangle]
    coordinates{ % plot 1 data set
      (35.15,0.58)
    }; 

    
    \addplot[only marks, mark options={scale=1.5}, mark=square]
    coordinates{ % plot 1 data set
      (46.87,0.588)
    }; 

  \end{axis}

\end{tikzpicture}

\end{tabular}
\captionsetup{font=small,labelfont=bf}
\vspace{-0.2cm}
\caption{Scatter plot illustrating the relation between the best-observed test accuracy on the CIFAR10 dataset (y-axis) and the amount of emitted CO$_2$e in grams (x-axis) with respect to the number of randomly selected clients. ``IID'' and ``non-IID'' correspond to the corpus partitioning strategy that is employed as described in Section \ref{sec:estimation}. It is nearly impossible to pick the right FL setup to maximize the performance and minimize the CO$_2$e emissions without an appropriate algorithm. However, the latter solution allows important CO$_2$e savings. Please note that the x-axis scale of the top-right plot is different due to a key increase in CO$_2$e emissions.}
\label{figcarbonefficiency}

\end{figure*}
%\vspace{-0.2cm}
